Towards Productionizing Subjective Search Systems

Existing e-commerce search engines typically support search only over objective attributes, such as price and locations, leaving the more desirable subjective attributes, such as romantic vibe and worklife balance unsearchable. We found that this is also the case for Recruit Group, which operates a wide range of online booking and search services, including jobs, travel, housing, bridal, dining, beauty, and where each service is among the biggest in Japan, if not internationally. We present our progress towards productionizing a recent subjective search prototype (OpineDB) developed by Megagon Labs for Recruit Group. Several components within OpineDB are enhanced to satisfy production demands, including adding a BERT language model pre-trained on massive hospitality domain review corpora. We also found that the challenges of productionizing the system are beyond enhancing the components. In particular, an important requirement in production-quality systems is to instrument a proper way of measuring the search quality, which is extremely tricky when the search results are subjective. This led to the creation of a high-quality benchmark dataset from scratch, involving over 600 queries by user interviews and a collection of more than 120,000 query-entity relevancy labels. Also, we found that the existing search algorithms do not meet the search quality standard required by production systems. Consequently, we enhanced the ranking model by fine-tuning several search algorithms and combining them under a learning-to-rank framework. The model achieves 5%-10% overall precision improvement and 90+% precision on more than half of the benchmark testing queries making these queries ready for AB-testing. While some enhancements can be immediately applied to other verticals, our experience reveals that benchmarking and fine-tuning ranking algorithms are specific to each domain and cannot be avoided.

==> model.tex <==
% %\newcommand{\db}{\mathcal{D}}
% \newcommand{\oa}{\mathsf{OA}}
% \newcommand{\sa}{\mathsf{SA}}
% \newcommand{\dom}{\mathsf{dom}}
% \newcommand{\od}{\mathsf{OD}}
% \newcommand{\sd}{\mathsf{SD}}
% \newcommand{\st}{\mathsf{ST}}
% \newcommand{\ex}{\mathsf{EX}}
% \newcommand{\et}{\mathsf{ET}}
% \newcommand{\at}{\mathsf{AT}}
% \newcommand{\op}{\mathsf{OP}}
% \renewcommand{\sp}{\mathsf{SP}}
% \newcommand{\aggr}{\mathsf{aggr}}


% \section{Data Model}
% \label{sec:datamodel}

% A relation in \system\ includes objective and subjective attributes. Informally, a subjective attribute represents an aggregate view of textual phrases extracted from reviews. 
% In this section we introduce {\em linguistic domains} that capture these phrases and {\em marker summaries} that represent the aggregates. 


% Consider the example of an attribute {\tt room\_cleanliness} in the domain of hotels. The raw data for this attribute exists in reviews and social media and consists of a wide variety of phrases such as 
% \begin{enumerate}\parskip=0pt
%     \item ``{\em The floor in my room was filthy dirty ...}'',
%     \vspace{-1mm}
%     \item ``{\em The room was clean, well-decorated and ...}'', or
%       \vspace{-1mm}
%     \item ``{\em Spotlessly clean and good location'}'.
% \end{enumerate}

% The challenge \system\ faces is to {\em aggregate} these phrases into a meaningful signal and to rank hotels appropriately in response to queries that may themselves include different linguistic phrases. The ability to aggregate linguistic phrases is one of the key aspects that distinguishes \system\ from text retrieval systems where ranking is typically based on similarity of unstructured text.


% To define an aggregation function, there needs to be a scale onto which the aggregation is performed. However, when dealing with text, we cannot always arrange the main landmarks in the domain into a linearly-ordered scale.  Hence, \system\ lets the schema designer define a set of {\em markers} in the domain that represent the points onto which we map the reviews. In our example, the markers might be a linear scale 
% $[$very\_clean, average, dirty, very\_dirty$]$ 
% for 
% room cleanliness and a set of markers for bathroom styles
% may be [old, standard, modern, luxurious], which
% is a set of categories (not a linear scale) that
% describes the different styles of bathroom.
%  \system\ maintains a {\em marker summary}, which is a view that aggregates the phrases from the reviews onto the markers.
%   Specifically,  \system\  computes a value representing the membership of each hotel for each marker. For example, the record
%  $[$very\_clean: 20, average: 70, dirty: 30, very\_dirty: 10$]$ for a hotel would represent that the hotel is closer to being a member of {\tt average} than to the other markers. As we see later, there  are different possible aggregation functions \system\ can use and the appropriate choice depends on the semantics of the attribute. 
%  At present, \system's marker summaries are histograms that tabulate the number of phrases of reviews closest to each marker.
%  Each marker summary also records features useful for query processing including the average sentiment score and the average phrase embedding vector.
% %  \wctan{number of reviews or number of phrases?} \yuliang{Decided to stay with ``phrases''. Need to do a global pass for consistency. }
%  %, and we describe the ones we use in %\system\ in %Section~\ref{sec:aggregation}. 
%  %\yuliang{change to ``the number of reviews centered at %each marker'' or 
%  %``the number of reviews being closest to each %marker''?}
 
%  In addition to aggregating the raw data, the marker summaries serve two other important goals. 
%  First, by aggregating the review data offline, query processing can be much more efficient. 
%  Accessing the raw data at query time would be prohibitively expensive. In our experiments,
%  query processing was accelerated by a factor of up
%  to  6.6x by only accessing the marker summaries. 
%  %\wctan{will be good if we can %reference our experiments here.}
%  %\yuliang{It is actually not too %expensive even if we perform online %aggregation,
%  %but we can talk about the speedup %here.}
%  Second, the markers enable the system designer to shape which important aspects of the reviews to highlight in the application.  Even though \system\ allows 
%  end users to specify arbitrary keywords in their query, 
%  markers can be useful for end users and applications
%  in gauging the range of linguistic terms that are supported by marker summaries.
 
 
%  We now describe each of the above components in detail.

% \smallskip
% \noindent
% {\bf Linguistic domains:} A {\em linguistic domain} is defined to be a set of short linguistic phrases 
% (which we refer to as {\em linguistic variations}) that describe a particular aspect of an object. 
% The linguistic domain allows \system\ to capture the different ways 
% of describing the cleanliness of a room.
% For example, \{ ``very clean'', ``pretty clean'', ``spotless'', ``average'', ``not dirty'', ``dirty'', ``stained carpet'', ``very dirty''...~\}
% is a linguistic domain for the cleanliness aspect of the room object. 
% %\yuliang{changed ``object'' to ``aspect of an object''. Please check.}
% %in the domain 
% %(e.g,. bathroom, hotel's service, etc.). 

% The linguistic domain is not enumerated in advance. \system\ bootstraps it by extracting phrases from the review data. 
% Phrases in reviews can express  opinions about an object directly (e.g., ``very clean room''), or 
% indirectly (e.g., ``the room has stained carpet''). 
% \system's extraction module supports both types of opinions.


% \smallskip
% \noindent
% {\bf Markers and Marker summaries:} A {\em marker summary} is defined over a linguistic domain and is a record type 
% $\mbox{Rcd}:[f_1, ..., f_k]$ 
% where \mbox{Rcd} is the name of the record,
% $f_i$ are names of {\em markers}, and the type for each field is assumed to be a number. There are two types of marker summaries: {\em linearly-ordered} or {\em categorical}. A linearly-ordered marker summary is one where $f_1, ..., f_k$ form a linear scale.  An example of a such a marker summary
% for room cleanliness over the linguistic domain described earlier is shown below.

% \vspace{-1mm}
% \begin{center}
% room\_cleanliness : [very\_clean, average, dirty, very\_dirty]   
% \end{center}
% \vspace{-1mm}

% \noindent
% A phrase can contribute {\em in part} to multiple markers of a linearly-ordered marker summary. For example, the phrase ``rooms are quite clean'' can contribute in equal proportions (0.5 each) 
% to the markers ``very\_clean'' and ``average''. 
% An example instance of the \\ room\_cleanliness marker summary is 
% $[$very\_clean: 90.5, average: 60.5, dirty: 30, very\_dirty: 20$]$. 
% We use the term ``marker summary'' to refer to either the record type or the record instance when the context is clear.
% %\wctan{added some discussions}

% Note that phrases in a linguistic domain do not always fall into a simple linearly-ordered scale of sentiment. For example, the fields we obtained by mining reviews from \url{booking.com} show that the quietness of a room may be described with words such as ``annoying'', ``peaceful'', ``very noisy'', ``traffic noise'', ``constant noise'', which do not follow a natural linear order.
% To handle such cases, we also allow for categorical marker summaries in \system.
% A categorical marker summary is one where no two markers form a linear
% scale. An example of a categorical marker summary is 
% \begin{center}
% style : [old, standard, modern, luxurious]   
% \end{center}
% \noindent
% A phrase can contribute {\em as a whole} to multiple markers in a categorical marker summary. For example,  ``extravagant old-fashioned bathrooms'' contributes
% to both ``old'' and ``luxurious'' (1 count each). 

% At present, we assume that a marker summary is either linearly-ordered or categorical.
% %hierarchical, negative phrases.
% %more recent reviews
% Of course, for each categorical marker such as ``luxurious'', there may be
% a linearly-ordered marker summary on the degree of ``luxuriousness''. As with any database design, it is the task of the schema designer to decide the appropriate  level of granularity to model the domain.
% In our context, \system\ assists 
%   her by clustering the linguistic domain (See Section~\ref{sec:domainmarkers} for details).
% %Each marker aggregate has an associated aggregation function to compute %how well each field represents the underlying reviews in terms of how %close is each review to a field of the record w.r.t. the linguistic %domain.
% %The reviews are then aggregated according to the marker summary (See Section \ref{sec:calculating-summaries}). 


% \smallskip
% \noindent
% {\bf Schema of a subjective database:} The schema of an \system\ application consists of three elements: (1)
% the main schema that is visible to the user and the application programmer,
% (2) the raw review data, and (3) the extractions of relevant phrases from the reviews from which we compute marker summaries. Parts (2) and (3) of the schema are intended to support queries that might qualify the reviews (e.g., consider only reviewers who have reviewed more than~10 hotels) and to support \system's ability to fall back on raw text when a query cannot be answered using the database schema. We discuss some of the details of these components of the schema in Section~\ref{sec:aggregation}. In what follows we focus on (1), which illustrates the main novel aspects of our data model. 

% \begin{figure}[t]
% %\centering
% %\includegraphics[width=.45\textwidth, height=5cm]{subjdbschema1.pdf}
% %\caption{A subjective database schema for hotels with four subjective %attributes {\tt room\_cleanliness}, {\tt style}, {\tt service}, and {\tt %vfm} along with their marker aggregates.}
% \begin{minipage}{0.55\textwidth}
% %\renewcommand{\arraystretch}{1.}
% \small
% \begin{tabbing}
% {\bf Hotels} 
% \begin{tabular}{|l|l|l|l|}
% \hline
% hotelname &  capacity &  address & price\_pn \\
% \hline
% \end{tabular}
% \end{tabbing}
% \normalsize

% \small
% \begin{tabbing}
% {\bf HRoomCleanliness} \=
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em room\_cleanliness} \\
% \hline
% \end{tabular} \\

% {\bf HBathroom} \>
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em style} \\
% \hline
% \end{tabular} \\

% {\bf HService} \>
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em service} \\
% \hline
% \end{tabular} \\

% {\bf HBed} \>
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em comfort} \\
% \hline
% \end{tabular}
% \end{tabbing}
% %\renewcommand{\arraystretch}{1.0}
% \normalsize
% \vspace{-1mm}
% %\smallskip
% \noindent
% \flushleft
% \small
% \vspace{-2mm}
% \underline{\bf Marker Summaries}\\
% \vspace{-2mm}
% \begin{tabbing}
% $\ast$ room\_cleanliness: \= [very\_clean, average, dirty, very\_dirty] \\
% $\ast$ style: \> [old, standard, modern, luxurious] \\
% $\ast$ service: \> [exceptional, good, average, bad, very\_bad] \\
% $\ast$ comfort: \> [very\_soft, soft, firm, very\_firm, ok, worn\_out]
% \end{tabbing}
% \normalsize
% \end{minipage}
% \vspace{-2mm}
% \caption{\small A subjective database schema for the hotel domain. Subjective attributes are prefixed with $\ast$.}
% \label{fig:subjdbschema}
% \vspace{-5mm}
% \end{figure}
% \normalsize


% \iffalse %%%

% \begin{figure*}[t]
% %\centering
% %\includegraphics[width=.45\textwidth, height=5cm]{subjdbschema1.pdf}
% %\caption{A subjective database schema for hotels with four subjective %attributes {\tt room\_cleanliness}, {\tt style}, {\tt service}, and {\tt %vfm} along with their marker aggregates.}
% \begin{minipage}{0.55\textwidth}
% \small
% \begin{tabbing}
% {\bf Hotels} 
% \begin{tabular}{|l|l|l|l|}
% \hline
% hotelname &  capacity &  address & price\_pn \\
% \hline
% \end{tabular}
% \end{tabbing}
% \normalsize

% \small
% \begin{tabbing}
% {\bf HRoomCleanliness} \=
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em room\_cleanliness} \\
% \hline
% \end{tabular} \\

% {\bf HBathroom} \>
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em style} \\
% \hline
% \end{tabular} \\

% {\bf HService} \>
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em service} \\
% \hline
% \end{tabular} \\

% {\bf HBed} \>
% \begin{tabular}{|l|l|}
% \hline
% hotelname & $\ast$ {\em comfort} \\
% \hline
% \end{tabular}
% \end{tabbing}
% \normalsize

% \smallskip
% \noindent
% \flushleft
% \small
% \underline{\bf Marker Summaries}\\
% \begin{tabbing}
% $\ast$ room\_cleanliness: \= [very\_clean, average, dirty, very\_dirty] \\
% $\ast$ style: \> [old, standard, modern, luxurious] \\
% $\ast$ service: \> [exceptional, good, average, bad, very\_bad] \\
% $\ast$ comfort: \> [very\_soft, soft, firm, very\_firm, ok, worn\_out]
% \end{tabbing}
% \normalsize
% \end{minipage}
% %\medskip
% %\hline 
% %\medskip
% \begin{minipage}{0.4\textwidth}
% \small
% \underline{\bf Extraction Relations and Source Reviews}

% {\bf RoomCleanlinessExtraction}\\
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% hotelname & reviewid & begin & end & phrase \\
% \hline
% \end{tabular}

% {\bf BathroomExtraction}\\
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% hotelname & reviewid & begin & end & phrase \\
% \hline
% \end{tabular}

% {\bf ServiceExtraction}\\
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% hotelname & reviewid & begin & end & phrase \\
% \hline
% \end{tabular}

% {\bf BedExtraction}\\
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% hotelname & reviewid & begin & end & phrase \\
% \hline
% \end{tabular}


% \smallskip
% \noindent
% \small
% {\bf SourceReviews}\\
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% hotelname & reviewid & author & date & text \\
% \hline
% \end{tabular}
% \end{minipage}
% \vspace{-2mm}
% \caption{A subjective database schema for the hotel domain. Subjective attributes are prefixed with $\ast$.}
% \vspace{-2mm}
% \label{fig:subjdbschema}
% \end{figure*}
% \normalsize

% \fi %%%%

% The schema that is visible to the user or the application is a finite sequence of relation schemas each
% of the following form: $R$($K$, $A_1$, $\ldots$, $A_n$)
% where $K$ is the key for $R$ (for simplicity, we assume it's a single attribute),  and  $A_1, \ldots, A_m$
% are a set of attributes.

% We distinguish between two types of attributes. 
% An {\em objective attribute} is an attribute whose value 
% is based on facts and is largely indisputable.
% In contrast, there is no ground 
% truth for the value of a {\em subjective attribute}.
% The value of a subjective attribute is ``influenced by or 
% based on personal beliefs or feelings, rather than based on 
% facts''.\footnote{\small{\url{https://dictionary.cambridge.org/us/dictionary/english/subjective}}}
% Figure~\ref{fig:subjdbschema} shows an example of a subjective database schema for the hotel domain.

% The type of a subjective attribute is a marker summary over a linguistic domain.
% The linguistic domain of the subjective attribute {\tt style}, for example,  is a set of phrases that may include \{ ``modern faucets'', ``old shower'', ``OK'', ``adequate'', ``luxurious bath towels'', ... \}. 
% As described earlier, the intuition is that the marker summary keeps a summary (e.g., histogram) of 
% the subjective phrases for that attribute w.r.t.\ the markers.

% %In our running example, the relations and marker %summaries in the left column of %Figure~\ref{fig:subjdbschema} are the ones %visible to the user.


% The key of the Hotels relation is {\tt hotelname} and it has three objective attributes, {\tt capacity}, {\tt address},
% and {\tt price\_pn}. There are four additional relations with the same key attribute
%  that contain subjective attributes. 
% The attributes {\tt room\_\-cleanliness}, {\tt style}, {\tt service}, {\tt comfort}
% are subjective 
% attributes of the relations HRoomCleanliness, HBathroom, HService, 
% and HBed
% respectively and their marker summaries are shown at the bottom of Figure~\ref{fig:subjdbschema}. 

% %The marker aggregates of the four subjective attributes are: \alon{I don't think we need 
% %{\tt service}: \\
% %$[$exceptional:\real, good:\real, average:\real, bad:\real, very\_bad:\real$]$ \\
% %{\tt vfm}: \\
% %$[$good\_price:\real, great\_value:\real, reasonable:\real, overpriced:\real$]$



% \iffalse %%%% SECOND and THIRD PART


% The second part of the schema, the  raw review data along with the date and author is stored in the following relation whose key is ({hotelname}, {reviewid}).

% \smallskip
% \noindent
% \small
% {\bf SourceReviews}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% hotelname & reviewid & author & date & text \\
% \hline
% \end{tabular}
% \smallskip
% \normalsize

% The third part of the schema includes the extractions from the reviews.
% The reviews are processed by an information extraction component whose goal is to find phrases describing the subjective attributes of the hotel. The 
% resulting facts are stored in the extraction relations. There
% is one extraction relation for each subjective attribute. The top 4 relations
% on the right side of Figure~\ref{fig:subjdbschema} shows the extraction relations
% for room cleanliness, bathrooms, service, and bed respectively.

% For each relation above and each hotel review, 
% the extractor retrieves all appropriate mentions in the text, if any, from the review, stores the span of tokens
% where the mention occurs with {\tt begin} and {\tt end} indicators and the span is stored under {\tt phrase}.
% An example of a tuple in the relation RoomCleanlinessExtraction is shown below:

% \smallskip
% \noindent
% \begin{tt}
% ("HolidayHotel", 128, "23", "25", "pretty clean")\smallskip
% \end{tt}

% \noindent
% Note that if the user desires to query only over recent reviews, such as those that are only made this year, new views of the extractors can be obtained by joining each of them
% with the SourceReviews relation on the key and placing a condition on {\tt date} where the year is required to be 2018.
% The marker summaries may be incrementally computed, 
% depending on the type of aggregation function used for computing the marker summary.
% Furthermore, any result returned can be supported with evidence from the reviews on why that result is returned.

% \fi %%%%%%%%%%%%%%%%%%%%%%%%%


% A core issue that \system\ needs to address is that of aggregating a large collection of linguistic phrases onto marker summaries, which we will describe in Section~\ref{sec:aggregation}. In what follows, we describe the query language
% of \system.

% \vspace{1mm}
% \noindent
% {\bf Query:~} The \system\ query language is essentially 
% SQL with the extra ability of specifying atomic conditions in natural language in the {\tt where} clause. 
% For the purposes of this paper, 
% we assume that an \system\ query consists of a single {\sf select}-{\sf from}-{\sf where} clause. 
% For example, assume that our hotel database is for hotels in London, then
% the query for hotels in London that cost less than 150 Euros per night, has clean rooms, and is good as a romantic getaway
% can be expressed as shown below:

% \renewcommand{\arraystretch}{1.1}
% \vspace{1mm}
% \begin{tabular}{p{.8cm}p{3in}}
% {\sf select} &  * \hspace{0.3cm}{\sf from} {\tt \ Hotels}\\
% {\sf where}  & {\tt price\_pn} $<$ 150 {\sf and}  \\
%              & ``{\em has really clean rooms}'' {\sf and} ``{\em is a romantic getaway}''
% \end{tabular}
% \vspace{1mm}
% \renewcommand{\arraystretch}{1.0}

% The {\tt where} clause is a 
% %conjunction or disjunction of %conditions. 
% logical expression over a set of conditions.
% The example above shows a conjunction of a condition on price and two 
% {\em query predicates} (or 
% {\em predicates} in short),
% which are conditions specified in natural language and they need not be phrases that occur in the reviews.
% The user can also directly query for clean rooms using the attribute {\tt room\_cleanliness} in the HRoomCleanliness relation. 
% However, to do so she will need to understand the exact semantics of the schema and specify the precise predicate, such as whether  ``clean rooms'' should be interpreted as ``very clean'', ``average'', ``dirty'' or ``very dirty'' rooms. 
% By extending the query language to accept natural language predicates, we can support a broader range of user interfaces to subjective databases. We will describe how
% \system\  automatically compiles the query predicates against the underlying schema.

% Of course, natural language queries can involve non-atomic conditions, but \system\ relies on techniques such as~\cite{zhong2017seq2sql} to decompose a complex query into atomic conditions. As such, we assume atomic query predicates throughout this paper.



% % \renewcommand{\arraystretch}{1.1}
% % \vspace{1mm}
% % {\sf select * from}
% % ({\sf select}  * \hspace{0.3cm}{\sf from} {\tt \ Hotels} {\sf where}  ``{\em has really clean room}'') \\
% % {\sf left outer join on} {\tt \ Hotels.street} $=$ {\tt \ Restaurants.street} \\
% % ({\sf select}  * \hspace{0.3cm}{\sf from} {\tt \ Restaurants} {\sf where}  ``{\em declicious Italian food}'')
% % \renewcommand{\arraystretch}{1.0}

% As we shall describe in Section~\ref{sec:life}, our subjective query interpreter compiles 
% the query predicate ``{\em has really clean rooms}'' into a predicate over the {\tt room\_cleanliness} attribute and
% the query predicate ``{\em is a romantic getaway}'' into a predicate over the {\tt service} and {\tt bathroom} attributes. 
% If the query predicate cannot be satisfactorily interpreted into a predicate over the existing schema, \system\ falls back to the source reviews to arrive at a ranked set of answers.


% % \yuliang{TODO: add a more complicated example showing the expressiveness of the language. }
% \smallskip
% \noindent
% \textbf{Benefits of a query language:} One of the 
% major advantages of \system\ is that subjective data can be queried declaratively, and therefore we can express complex queries. For example, the semantics of the following query is well defined: 
% \emph{``find hotels with clean room based on reviews after 2010''}. Another important example is queries involving joins, such as 
% \emph{``find a hotel with a lively bar on the same street as a cafe with a relaxing atmosphere.''} 
% (Figure \ref{fig:sql_example}, we leave the discussion of the join semantics to future work).
% Being implemented on an RDBMS, \system\ is also able to leverage any query optimization capability of
% the underlying engine to boost the querying performance. 
% \vspace{-2mm}
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.46\textwidth]{sql_example.pdf}
%     \vspace{-3mm}
%     \caption{\small{An example of an \system\ query with joins.}}
%     \vspace{-2mm}
%     \label{fig:sql_example}
% \end{figure}

% Next, we describe how \system\ processes queries.
% Although we continue to exemplify our technical discussions with examples from the hotel domain, the techniques we develop are not dependent on a particular domain. In fact, we have conducted our experiments in Section~\ref{sec:experiments} on two domains: 
% hotels and restaurants.




==> related-minimum.tex <==
% \section{Related work}\label{sec:related}

% The fields of sentiment analysis and opinion mining~\cite{liu2012sentiment} have developed techniques for extracting subjective data from text. While sentiment analysis tries to decide whether a particular text is positive or negative about an object or an aspect of an object, opinion mining aims to summarize a large collection of sentiments in a way that is informative to the user. %In contrast, \system\ motivates the need to incorporate subjective opinion data into a general data management system, and addresses the challenges involved in doing so.
% %
% %
% %The first of these challenges is to answer 
% %complex queries over opinion data, and in particular queries that involve multiple subjective attributes and combining subjective and objective attributes.  In addition, complex queries may restrict the reviews of interest by filtering only reviews of a certain nature (e.g., prolific reviewers, or reviewers that agree with the user's taste).  To the best of our knowledge, answering complex queries over review data has not been 
% %considered in previous work.
% %
% %The second challenge \system\ faces is to enable the application designer to apply domain semantics to the management and querying of review data. For example, the way opinions about a particular attribute are aggregated may depend on its semantics (e.g., aggregating an attribute that highly sensitive to time should
% %give higher weight to more recent reviews).  In addition, the designer may also want to tailor which distinctions in the data to highlight. For example, instead of merely having a positive or negative opinion about bathroom cleanliness, the designer may choose to consider the distinctions about the cleanliness of the shower or the water pressure. We introduce the concept of marker summaries to provide the designer such flexibility. 
% %
% In contrast, \system\ enables the application designer to incorporate subjective opinion data into a general data management system, and \system\ offers users to issue complex queries that involve multiple subjective predicates.

% %\system\ also leverages previous work on extracting subjective aspects from reviews in order to construct the schema of a subjective database.  This task itself relates to aspect extraction and opinion lexicon construction that are well-studied in opinion mining~\cite{liu2012sentiment, absa}. Hu and Liu~\cite{hu2004aaai} proposed to extract product aspects from reviews using language rules. LocLDA~\cite{brody10hltnaacl} and BTM~\cite{yan13www} explored topic models to discover coherent aspects. ABAE~\cite{he17acl} developed neural approach to further improve the quality of extracted aspects. To generate opinion words for an aspect, there are two popular threads of algorithms. Dictionary-based approaches~\cite{hu2004aaai, liu2012sentiment, tai2013iiwas, vicente2014eacl} utilize public synonym or antonym dictionaries to bootstrap a set of opinion words. Corpus-based approaches~\cite{qiu2011coling, liu2012sentiment, rothe2016naacl, fast2016chi, hamilton2016emnlp, chen2018coling} target specific domains and discover domain-specific opinion words. 
% %\system\ follows a similar approach which bootstraps the linguistic domains using 
% %domain-specific word vectors trained with word2vec~\cite{mikolov2013nips}. 
% %In addition, \system\ involves a human in the loop in the process of extracting the linguistic domains in order to ensure high quality. 

% \system\ also leverages previous work on extracting subjective aspects from reviews in order to construct the schema of a subjective database.  This task itself relates to aspect extraction~\cite{hu2004aaai, brody10hltnaacl, yan13www, he17acl} and opinion lexicon construction~\cite{hu2004aaai, liu2012sentiment, tai2013iiwas, vicente2014eacl, qiu2011coling, liu2012sentiment, rothe2016naacl, fast2016chi, hamilton2016emnlp, chen2018coling} that are well-studied in opinion mining~\cite{liu2012sentiment, absa}.  \system\ follows a similar approach which bootstraps the linguistic domains using 
% domain-specific word vectors trained with word2vec~\cite{mikolov2013nips}. 
% In addition, \system\ involves a human in the loop in the process of extracting the linguistic domains in order to ensure high quality. 

% %To the best of our knowledge, opinion-based entity ranking~\cite{genesan2012infretr, makris2014webist} 
% %are the only works that considered subjective queries 
% %and utilized reviews for ranking entities. Specifically, \cite{genesan2012infretr} concatenated all the reviews into a single review document for every entity. On receiving query text, they calculated a matching score for every review document using a retrieval model such as BM25. 
% %However, they did not aggregate the reviews or support complex queries like \system. Trummer et al.~\cite{DBLP:conf/sigmod/TrummerHLSG15} note that many queries to web search engines are of subjective nature and consider the problem of aggregating subjective opinions about (entity, attribute) pairs (e.g., cute animals). Aroyo and Welty~\cite{DBLP:journals/aim/AroyoW15} note that in the process of annotating training data for machine learning, there are several fallacies in assuming that there is an objective truth for the annotations. They develop a measure that supports differing subjective opinions from annotators. Subjective databases are different from probabilistic databases~\cite{DBLP:series/synthesis/2011Suciu} in that the latter still assume that there is an objective ground truth but it is not known to the database. 

% To the best of our knowledge, opinion-based entity ranking~\cite{genesan2012infretr, makris2014webist} 
% are the only works that considered subjective queries 
% and utilized reviews for ranking entities. %Specifically, \cite{genesan2012infretr} concatenated all the reviews into a single review document for every entity. On receiving query text, they calculated a matching score for every review document using a retrieval model such as BM25. 
% However, they did not aggregate the reviews or support complex queries like \system. Trummer et al.~\cite{DBLP:conf/sigmod/TrummerHLSG15} note that many queries to web search engines are of subjective nature .%and consider the problem of aggregating subjective opinions about (entity, attribute) pairs (e.g., cute animals). 
% Aroyo and Welty~\cite{DBLP:journals/aim/AroyoW15} note that in the process of annotating training data for machine learning, there are several fallacies in assuming that there is an objective truth for the annotations. %They develop a measure that supports differing subjective opinions from annotators. 
% Subjective databases are different from probabilistic databases~\cite{DBLP:series/synthesis/2011Suciu} in that the latter still assume that there is an objective ground truth but it is not known to the database.
% %
% %\system\ uses a variant of fuzzy logic to match query terms against items in the database and to combine the scores of multiple query terms. Fuzzy logic has been used in a myriad of applications in AI,
% % control theory, and even databases with the capability of reasoning with vague and/or partial predicates 
% %like ``warm'' or ``fast'' \cite{zadeh1996fuzzy,klir1995fuzzy,fagin1996combining}.
% %Fuzzy logic generalizes the classic boolean logic with
% %the ``degree of truth'' which can take real values from $0$ to $1$.
% %In contrast to previous work where fuzzy logic is used to reason about  ``partial truth''
% %or subjective perception of objective attributes like temperatures or speed,  
% %our work considers processing queries on data that is itself subjective.
% %
% %The problem of building natural language interfaces to databases is a long standing one~\cite{NLI2DB} and more recent work (e.g.,~\cite{IyerKCKZ17, LiJ16, PopescuEK03, Poon13}) has focused on learning how to parse natural language into a corresponding semantic form (e.g., SQL) based on examples of pairs of such. \system\ does not translate natural language into SQL. Instead, it supports query terms, which are short phrases, that are already embedded in an SQL-like query. Furthermore, the main focus of these works is on parsing objective queries but \system\ interprets and evaluates subjective queries. 
% %
% Subjective queries do not have ground-truth answers, \system\ presents a way to express such queries in SQL~\cite{IyerKCKZ17, LiJ16, PopescuEK03, Poon13} and process them using fuzzy logic\cite{zadeh1996fuzzy,klir1995fuzzy,fagin1996combining}. 



==> related-short.tex <==
% \section{Related work}\label{sec:related}

% The fields of sentiment analysis and opinion mining~\cite{liu2012sentiment} have developed techniques for extracting subjective data from text. While sentiment analysis tries to decide whether a particular text is positive or negative about an object or an aspect of an object, opinion mining aims to summarize a large collection of sentiments in a way that is informative to the user. In contrast, \system\ motivates the need to incorporate subjective opinion data into a general data management system, and addresses the challenges involved in doing so.

% The first of these challenges is to answer 
% complex queries over opinion data, and in particular queries that involve multiple subjective attributes and combining subjective and objective attributes.  In addition, complex queries may restrict the reviews of interest by filtering only reviews of a certain nature (e.g., prolific reviewers, or reviewers that agree with the user's taste).  To the best of our knowledge, answering complex queries over review data has not been 
% considered in previous work.

% The second challenge \system\ faces is to enable the application designer to apply domain semantics to the management and querying of review data. For example, the way opinions about a particular attribute are aggregated may depend on its semantics (e.g., aggregating an attribute that is highly sensitive to time should
% give higher weight to more recent reviews).  In addition, the designer may also want to tailor which distinctions in the data to highlight. For example, instead of merely having a positive or negative opinion about bathroom cleanliness, the designer may choose to consider the distinctions about the cleanliness of the shower or the water pressure. We introduce the concept of marker summaries to provide the designer such flexibility. 

% %\system\ also leverages previous work on extracting subjective aspects from reviews in order to construct the schema of a subjective database.  This task itself relates to aspect extraction and opinion lexicon construction that are well-studied in opinion mining~\cite{liu2012sentiment, absa}. Hu and Liu~\cite{hu2004aaai} proposed to extract product aspects from reviews using language rules. LocLDA~\cite{brody10hltnaacl} and BTM~\cite{yan13www} explored topic models to discover coherent aspects. ABAE~\cite{he17acl} developed neural approach to further improve the quality of extracted aspects. To generate opinion words for an aspect, there are two popular threads of algorithms. Dictionary-based approaches~\cite{hu2004aaai, liu2012sentiment, tai2013iiwas, vicente2014eacl} utilize public synonym or antonym dictionaries to bootstrap a set of opinion words. Corpus-based approaches~\cite{qiu2011coling, liu2012sentiment, rothe2016naacl, fast2016chi, hamilton2016emnlp, chen2018coling} target specific domains and discover domain-specific opinion words. 
% %\system\ follows a similar approach which bootstraps the linguistic domains using 
% %domain-specific word vectors trained with word2vec~\cite{mikolov2013nips}. 
% %In addition, \system\ involves a human in the loop in the process of extracting the linguistic domains in order to ensure high quality. 

% \system\ also leverages previous work on extracting subjective aspects from reviews in order to construct the schema of a subjective database.  This task itself relates to aspect extraction~\cite{hu2004aaai, brody10hltnaacl, yan13www, he17acl} and opinion lexicon construction~\cite{hu2004aaai, liu2012sentiment, tai2013iiwas, vicente2014eacl, qiu2011coling, liu2012sentiment, rothe2016naacl, fast2016chi, hamilton2016emnlp, chen2018coling} that are well-studied in opinion mining~\cite{liu2012sentiment, absa}.  \system\ follows a similar approach which bootstraps the linguistic domains using 
% domain-specific word vectors trained with word2vec~\cite{mikolov2013nips}. 
% In addition, \system\ involves a human in the loop in the process of extracting the linguistic domains in order to ensure high quality. 

% To the best of our knowledge, opinion-based entity ranking~\cite{genesan2012infretr, makris2014webist} 
% are the only works that considered subjective queries 
% and utilized reviews for ranking entities. %Specifically, \cite{genesan2012infretr} concatenated all the reviews into a single review document for every entity. On receiving query text, they calculated a matching score for every review document using a retrieval model such as BM25. 
% However, that work did not aggregate the reviews or support complex queries like \system. 
% Trummer et al.~\cite{DBLP:conf/sigmod/TrummerHLSG15} note that many queries to web search engines are of subjective nature and consider the problem of aggregating subjective opinions about (entity, attribute) pairs (e.g., cute animals). Aroyo and Welty~\cite{DBLP:journals/aim/AroyoW15} note that in the process of annotating training data for machine learning, there are several fallacies in assuming that there is an objective truth for the annotations. They develop a measure that supports differing subjective opinions from annotators.
% %They develop a measure that supports differing subjective opinions from annotators. 
% Subjective databases are different from probabilistic databases~\cite{DBLP:series/synthesis/2011Suciu} in that the latter still assume that there is an objective ground truth but it is not known to the database. 

% \system\ explores a variant of fuzzy logic to match query terms against items in the database and to combine the scores of multiple query terms. Fuzzy logic has been used in a myriad of applications in AI,
%  control theory, and even databases with the capability of reasoning with vague and/or partial predicates 
% like ``warm'' or ``fast'' \cite{zadeh1996fuzzy,klir1995fuzzy,fagin1996combining}.
% %Fuzzy logic generalizes the classic boolean logic with
% %the ``degree of truth'' which can take real values from $0$ to $1$.
% In contrast to previous work where fuzzy logic is used to reason about  ``partial truth''
% or subjective perception of objective attributes like temperatures or speed,  
% our work considers processing queries on data that is itself subjective.

% The problem of building natural language interfaces to databases is a long standing one~\cite{NLI2DB} and more recent work (e.g.,~\cite{IyerKCKZ17, LiJ16, PopescuEK03, Poon13}) 
% has focused on learning how to parse natural language into a corresponding semantic form (e.g., SQL) 
% based on examples of pairs of such. 
% \system\ does not translate natural language into SQL. Instead, it supports query predicates, which are short phrases, that are already embedded in an SQL-like query.
% Furthermore, the main focus of these works is on parsing objective queries but 
% \system\ interprets and evaluates subjective queries. 


